Topological $k$-metrics

Metric spaces $(X, d)$ are ubiquitous objects in mathematics and computer science that allow for capturing (pairwise) distance relationships $d(x, y)$ between points $x, y \in X$. Because of this, it is natural to ask what useful generalizations there are of metric spaces for capturing "$k$-wise distance relationships" $d(x_1, \ldots, x_k)$ among points $x_1, \ldots, x_k \in X$ for $k > 2$. To that end, G\"{a}hler (Math. Nachr., 1963) (and perhaps others even earlier) defined $k$-metric spaces, which generalize metric spaces, and most notably generalize the triangle inequality $d(x_1, x_2) \leq d(x_1, y) + d(y, x_2)$ to the "simplex inequality" $d(x_1, \ldots, x_k) \leq \sum_{i=1}^k d(x_1, \ldots, x_{i-1}, y, x_{i+1}, \ldots, x_k)$. (The definition holds for any fixed $k \geq 2$, and a $2$-metric space is just a (standard) metric space.) In this work, we introduce strong $k$-metric spaces, $k$-metric spaces that satisfy a topological condition stronger than the simplex inequality, which makes them "behave nicely." We also introduce coboundary $k$-metrics, which generalize $\ell_p$ metrics (and in fact all finite metric spaces induced by norms) and minimum bounding chain $k$-metrics, which generalize shortest path metrics (and capture all strong $k$-metrics). Using these definitions, we prove analogs of a number of fundamental results about embedding finite metric spaces including Fr\'{e}chet embedding (isometric embedding into $\ell_{\infty}$) and isometric embedding of all tree metrics into $\ell_1$. We also study relationships between families of (strong) $k$-metrics, and show that natural quantities, like simplex volume, are strong $k$-metrics.

==> general-cuts.tex <==
\section{Cuts}

\begin{definition}[Volume $k$-metrics]
\label{def:volume_norms}
Let $X$ be a finite set of points, and let $d$ be a function on $k$-tuples of $X$, and let $||\cdot||$ be any vector norm.
We say that $(X, d)$ belongs to the \EMPH{volume metric} ${\cal V}(k, \R^m, ||\cdot||)$ if there exists a map $f:X\rightarrow \R^m$, such that for any $k$-tuple $x_1, \ldots, x_k \in X$ (possibly with duplicated elements), we have
\[
d(x_1, \ldots, x_k) = \left|\left| 
    \left(
        \text{vol}_{k-1}\left(\pi(f({x}_1)),\dots, \pi(f({x}_{k}))\right)
    \right)_{\pi\in\Pi}
\right|\right|
\ \text{,}
\]
where $\Pi$ is the set of all $\binom{m}{k}$ orthogonal projections onto $(k-1)$-dimensional axis-aligned hyperplanes in $\R^m$, and $\vol_{k-1}$ is the $(k-1)$-volume of $k$-simplices in $\R^{k-1}$, defined above.
\end{definition}


\begin{definition}[Cut $2$-Pesudometrics]
For $x,y,z\in[0,1]$, $x\leq y$ we define a cut pesudometric (often referred to simply as a cut metric) $d_z(x,y)$ as:

\begin{equation*}
d_z(x,y)=\begin{cases}
          1 \quad &x \leq z \leq y \And x\neq y\\
          1 \quad &y \leq z \leq x \And x\neq y\\
          0 \quad &\text{otherwise} \\
     \end{cases}
\end{equation*}
\end{definition}
This is a different formulation of a cut pesudometric than usual - normally we would construct a cut $f$ which assigns value 1 to every point in $[z,1]$ and 0 to the rest, with $|f(x)-f(y)|$ inducing the cut pesudometric. Note also that under the usual construction $(\forall w<z\, d_z(w,z) =1)$ xor $(\forall w>z\, d_z(w,z) =1)$, whereas with this formulation both are true.

We also limit ourselves to the special case of a cut over the unit interval. While cut metrics are defined in general, most of our results require a bounded domain. Larger domains require an additional scaling factor of the n-volume (here length) of the space. These results also hold for bounded spaces of other sizes after dividing by this scaling factor.
Cut metrics have a number of properties that lend themselves to a number of proofs. In generalizing metric input dimensions we seek to define similar 'cut pesudometrics' for other numbers of inputs while maintaining properties analogous to the following:
\begin{proposition}
$\forall x,y\in [0,1],\, |x-y|=\mathbb{E}_{z\in[0,1]}(d_z(x,y))$
That is, the expected value of a pair of points under a random cut pesudometric equals their distance.
\end{proposition}
\begin{proposition}
Any $2$-metric in $\ell_1$ in $[0,1]^m$ can be decomposed into a convex combination of cut pesudometrics. $$\mathbb{E}_\delta(\delta(x,y))=\frac{1}{m}\sum_{i=1}^m |x\cdot e_i-y\cdot e_i|=||x-y||_1/m$$
Where $\delta$ is chosen uniformly at random from the space of possible cuts on every axis.
\end{proposition}

\subsection{General Cuts}

Recalling prop \wnote{expected values and decompostion}, we would like to extend these properties to our generalized metrics in $\R^n$. With this motivation, we define our generalized n-cut as follows
\begin{definition}[$n$-cut metric]
For $x, a_1, \dots, a_n \in [0, 1]^{n-1}$, we define the $n$-cut metric
\[
d_x(a_1,a_2,\dots,a_n) :=
\begin{cases}
1 & \text{if $x \in \conv(a_1,a_2,\dots,a_n)$} \ \text{,} \\
0 & \text{otherwise} \ \text{.}
\end{cases}
\]
\end{definition}
\begin{lemma}
The $n$-cut metric in the unit n-1 cube $d_x:[0,1]^{n(n-1)}\to \{0,1\}$, as defined above, is an n-metric
\end{lemma}
\begin{proof}
\begin{enumerate}
    \item [0] Since the only values $d_x$ assigns are 0 and 1, this holds
    \item [1] By our definition, if the $a_i$ lie in an $n-2$ dimensional subset (i.e. collinear, coplanar, ect.) then the tuple has value 0.
    \item [2] Convex hulls are insensitive to permutation of inputs
    \item [3] We want to show that for an arbitrary point $b\in [0,1]^{n-1}$, $d_x(a_1,\dots,a_n)\leq d_x(b,a_2,\dots,a_n)+d_x(a_1,b,a_3,\dots,a_n)+\dots+d_x(a_1,\dots,a_{n-1},b)$. If b lies in the hull (including on its boundary) this is trivial, since the new hulls cover the original, thus at least one must contain x. Thus it remains to show that this holds for b outside the hull. Since convex hulls are closed, the line connecting an arbitrary point b to the cut point x will intersect at least 2 faces, one of which is further from w than z. The convex hull of the vertices of this face and w will thus necessarily contain x, which ensure that the triangle inequality holds. (Note that if the line intersects with a subspace of dimension $<n-1$ then we can select any face which contains it.)
\end{enumerate}
\end{proof}

Since the odds of a random point falling within a given convex hull is the n-volume taken up by it, we have:
\begin{lemma}
$\forall x_1,x_2,\dots,x_n\in [0,1]^{n-1},\,\text{vol}_{k-1}(\text{conv}(x_1,x_2,\dots,x_n)=\mathbb{E}_z\in{[0,1]^{n-1}}(d_z(x_1,x_2,\dots,x_n))$
\end{lemma}

We can think of these as a norm on the volumes of the lower dimensional projections of the polytope defined by the $x_i$.
While it is obvious that these have properties 1,2, and 4 of a vector norm, scalar multiplication brings some added complexity.

For conventional norms we have $||n\vec{x}||=|n|\cdot||\vec{x}||$, and for area norms we have 
\hnote{As I think we discussed in person at some point, this is wrong. Volume scales with dimension. That is, if $K$ is an $n$-dimensional measurable set and $c > 0$ then $\vol_n(cK) = c^n \vol_n(K)$. There's no factor of $2$ in the $2$-dimensional case.} $d(na,nb,nc)=(n^2/2)d(a,b,c)$ \wnote{imagine there's a nice pattern - ie $n^{k-1}/(k-1)!$ $n$-dimensional volume scales exponentially in $n$!}

This definition allows us to extend \wnote{prev prop} as follows:
\begin{theorem} [Decomposition into $n$-Cuts]
We can express any finite metric on a $d_{n,1}$ norm ($n>1$) as the convex combination of n-cuts

\end{theorem}
\begin{proof}
$$\mathbb{E}_\delta(\delta(u_1,u_2,\dots, u_n))=\frac{1}{N^n}\sum_{\pi} \text{volume}(\text{conv}(\pi(u_1),\pi(u_2),\dots,\pi(u_n)))=N^{-n}d_{n,1}(u_1,u_2,\dots, u_n)$$
where $\pi$ is projection onto n-1 random axes.
\end{proof}
